Runtime Advocates: A Persona-Driven Framework for Requirements@Runtime Decision Support

Complex systems, such as small Uncrewed Aerial Systems (sUAS) swarms dispatched for emergency response, often require dynamic reconfiguration at runtime under the supervision of human operators. This introduces human-on-the-loop requirements, where evolving needs shape ongoing system functionality and behaviors. While traditional personas support upfront, static requirements elicitation, we propose a persona-based advocate framework for runtime requirements engineering to provide ethically informed, safety-driven, and regulatory-aware decision support. Our approach extends standard personas into event-driven personas. When triggered by events such as adverse environmental conditions, evolving mission state, or operational constraints, the framework updates the sUAS operator's view of the personas, ensuring relevance to current conditions. We create three key advocate personas, namely Safety Controller, Ethical Governor, and Regulatory Auditor, to manage trade-offs among risk, ethical considerations, and regulatory compliance. We perform a proof-of-concept validation in an emergency response scenario using sUAS, showing how our advocate personas provide context-aware guidance grounded in safety, regulatory, and ethical constraints. By evolving static, design-time personas into adaptive, event-driven advocates, the framework surfaces mission-critical runtime requirements in response to changing conditions. These requirements shape operator decisions in real time, aligning actions with the operational demands of the moment.

==> 6_Future_Work.tex <==
% Moved to conclusion
\section{Future Work}
In additional work we plan to fully evaluate RAVEN in a series of user-studies conducted in a high-fidelity simulation environment and in real-world environments with end-users. We will assess the usefulness and trustworthiness of the advocates to diverse users, and will compare our current push-model (where advice is dynamically pushed to the user in a similar format to warning messages, to a pull-model (in which users can seek advice upon demand), and to various hybrid models.

We will also extend the advocates themselves in several ways. First, by considering additional types of advocates that might be relevant across the sUAS and other domains, and second, by enhancing the accuracy and usefulness of current advocates, for example, by enhancing the pipeline with machine-learning techniques to improve filtering of recommendations, and by integrating retrieval-augmented generation (RAG) methods, richer world state representations, and potentially graphical inputs to improve the reliability and fidelity of persona prompting in dynamic environments.
